OliVe: Accelerating Large Language Models via Hardware-friendly Outlier-Victim Pair Quantization

Transformer-based large language models (LLMs) have achieved great success with the growing model size. LLMs' size grows by $240\times$ every two years, which outpaces the hardware progress and makes model inference increasingly costly. Model quantization is a promising approach to mitigate the widening gap between LLM size and hardware capacity. However, the existence of outliers, values with significant magnitudes, in LLMs makes existing quantization methods less effective. Prior outlier-aware quantization schemes adopt sparsity encoding techniques to separate outliers from normal values where the process requires global coordination (e.g., a global sparsity coordination list). This incurs complex encoding/decoding hardware logics and an extra orchestration controller for the computation between outlier and normal values. As such, it is not hardware-efficient and hence only achieves sub-optimal quantization benefits. We propose OliVe, an algorithm/architecture co-designed solution that adopts an outlier-victim pair (OVP) quantization and handles outlier values locally with low hardware overheads and high performance gains. The key insight of OliVe is that outliers are important while the normal values next to them are not. Thus those normal values (called victims) can be sacrificed to accommodate outliers. This enables a memory-aligned OVP encoding scheme, which can be efficiently integrated to the existing hardware accelerators like systolic array and tensor core. As a result, OliVe-based accelerator surpasses the existing outlier-aware accelerator, GOBO, by 4.5$\times$ speedup and 4.0$\times$ energy reduction, respectively, with a superior model accuracy.

==> tex/background.tex <==
\vspace*{0.3cm}
\section{Background}
\label{sec:background}
This section presents relevant background on Transformer architecture and recent large language model. We then describe the outlier-ware quantization and mixed precision, which has been widely studied to reduce the memory and computation cost of Transformer models.
\begin{table}[t]
    \ra{1.0}
    \centering
    \begin{tabular}{c|c|c}
        \textbf{Model} &
      \textbf{Parameter (Billion)} &
      \textbf{Year}  \\ \Xhline{1.2pt}

      \textbf{GPT} & 0.117 & 2018 \\ \hline
    
      \textbf{BERT$_{large}$} & 0.34 & 2018 \\ \hline

      \textbf{RoBERTa$_{large}$} & 0.355 & 2019 \\ \hline
  
      \textbf{GPT-2} & 1.5 & 2019  \\ \hline

      \textbf{T5} & 11 & 2019  \\ \hline

      \textbf{GPT-3} & 175 & 2020  \\ \hline

      \textbf{OPT} & 175 & 2022  \\ \hline

      \textbf{BLOOM} & 176 & 2022  \\

    \end{tabular} 
\caption{The parameter of transformer model.}
% \vspace{-5pt}
\label{tab:transformer_model}
\end{table}

\subsection{Transformer}
Transformer-based models achieve superior performance in the natural language field~\cite{}. There are decoder, encoder, and encoder-decoder architectures in transformer-based models. The encoder maps the initial sequence to a set of tokens, and tokens are further converted into vectors. Given the outputs, the decoder will generate a sequence of symbols. The initial transformer architecture transforms input sentences into output sentences by encoder and decoder, and is generally used for machine translation. Pre-trained language models have become the indispensable toolkit for NLP researchers. Google's BERT~\cite{devlin2018bert} (Bidirectional Encoder Representation from Transformer) have been widely used in natural language understanding task. BERT is pre-trained on unlabeled data over different pre-training tasks, and then the pre-trained model is fine-tuned by labeled data from the downstream tasks. GLUE~\cite{wang2018glue} and SQuAD~\cite{rajpurkar-etal-2016-squad} are commonly used to evaluate the performance of BERT-like models. Generative language models, such as GPT-2~\cite{radford2019language}, GPT-3~\cite{brown2020language}, OPT~\cite{zhang2022opt}, with a left-to-right architecture, use the previous information to predict future tokens. Specifically speaking, the generative language models output results token-by-token and follow the decoder structure of the transformers. This work explores both BERT-like and GPT-like architectures.

The trend of current transformer models is that more layers bring more powerful performance. Table \ref{tab:transformer_model} shows the size of some language models in different years. More and more institutes are releasing their large pre-trained language models at the 100 billion level~\cite{brown2020language, zhang2022opt, chowdhery2022palm, scao2022bloom}. The GPT-like model with 175 billion~\cite{brown2020language, zhang2022opt} parameters has proven to be impressively successful on a variety of natural language tasks. However, large-scale models dramatically increase the overhead of data transfers, memory accesses, storage, and computations. The growth of model size far outpaces the hardware performance improvement. Thus, the compression and quantization of large-scale models are of great interest.
 
\subsection{Quantization}
Quantization technique reduces the bit precision of weight and activation tensors, leading to lower memory footprint and more efficient computing. Lower-bit quantization has a trade-off between range and resolution for the representation. Post-training quantization (PTQ) and quantization-aware quantization (QAT) are two popular quantization methods. QAT allows the model to adapt to quantization noise due to fine-tuning. Thus, QAT can find a more optimal solution for a model than PTQ. However, it requires a time-consuming processing, especially for large language models. OPT-175B was continuously trained on 992 \textit{80GB A100 GPUs} for about 33 days. BLOOM-176B was trained for 3.5 months on 384 \textit{80GB A100 GPUs}. As we can see, QAT is unfeasible even for language models at billion scales. PTQ is very effective and fast to implement since it converts the original pre-trained FP32 model directly into a lower-bit model without the training data and pipeline. Thus, PTQ can overcome the overhead problem in large language model quantization. \textbf{\proj{}} explores the both QAT and PTQ results on BERT-like models, as well as the PTQ results on billion-level generative language models.


\subsection{Outlier-aware quantization}
Outlier value has a significant impact on quantization precision, especially for large-scale model. Clipping outlier value to a relatively small range may cause a large perturbation to the network, which may lead to model failure. Outlier-aware quantization (OLAccel)~\cite{park2018energy} divides the value in a tensor into outlier and normal regions. The values in outlier region can be represented by high precision and in normal region are compressed to lower bits. LLM.int8()~\cite{dettmers2022llm} exploits vector-wise quantization to confine the effect of outlier values to finer granularity and provide a more appropriate scale than tensor-wise quantization. GOBO~\cite{zadeh2020gobo} compressed the vast majority of weights to 3b or 4b indexes into a dictionary. The very few — typically less 0.1\% per layer — outlier values remain as-is.


The additional noise of quantization leads degradation in the large-scale models. 

\subsection{Mixed Precision and Mixed Data Type}


% \lipsum[1-4]
